Whodunit? Learning to Contrast for Authorship Attribution

Authorship attribution is the task of identifying the author of a given text. The key is finding representations that can differentiate between authors. Existing approaches typically use manually designed features that capture a dataset's content and style, but these approaches are dataset-dependent and yield inconsistent performance across corpora. In this work, we propose \textit{learning} author-specific representations by fine-tuning pre-trained generic language representations with a contrastive objective (Contra-X). We show that Contra-X learns representations that form highly separable clusters for different authors. It advances the state-of-the-art on multiple human and machine authorship attribution benchmarks, enabling improvements of up to 6.8% over cross-entropy fine-tuning. However, we find that Contra-X improves overall accuracy at the cost of sacrificing performance for some authors. Resolving this tension will be an important direction for future work. To the best of our knowledge, we are the first to integrate contrastive learning with pre-trained language model fine-tuning for authorship attribution.

==> deleted/acl_arr_2_coling <==
% % This must be in the first 5 lines to tell arXiv to use pdfLaTeX, which is strongly recommended.
% \pdfoutput=1
% % In particular, the hyperref package requires pdfLaTeX in order to break URLs across lines.

% \documentclass[11pt]{article}

% % Remove the "review" option to generate the final version.
% \usepackage[review]{acl}

% % Standard package includes
% \usepackage{times}
% \usepackage{latexsym}
% \usepackage{cite}
% \usepackage{amsmath,amssymb,amsfonts}
% \usepackage{subcaption}
% \usepackage{algorithmic}
% \usepackage{graphicx}
% \usepackage{textcomp}
% \usepackage{xcolor}
% \usepackage{textcomp}
% \usepackage{mathtools}  
% \usepackage{dsfont}
% \usepackage{hyperref}
% \usepackage{booktabs}
% \usepackage{multirow}

% \DeclareMathOperator*{\E}{\mathbb{E}}

% % import all macros
% \input{macros}

% % For proper rendering and hyphenation of words containing Latin characters (including in bib files)
% \usepackage[T1]{fontenc}
% % For Vietnamese characters
% % \usepackage[T5]{fontenc}
% % See https://www.latex-project.org/help/documentation/encguide.pdf for other character sets

% % This assumes your files are encoded as UTF8
% \usepackage[utf8]{inputenc}
% \usepackage{enumitem}
% % This is not strictly necessary, and may be commented out,
% % but it will improve the layout of the manuscript,
% % and will typically save some space.
% \usepackage{microtype}

% % If the title and author information does not fit in the area allocated, uncomment the following
% %
% %\setlength\titlebox{<dim>}
% %
% % and set <dim> to something 5cm or larger.

% % \makeatletter
% % \setlength{\@fptop}{0pt}
% % \makeatother

% \title{Whodunit? Learning to Contrast for Authorship Attribution}

% % Author information can be set in various styles:
% % For several authors from the same institution:
% % \author{Author 1 \and ... \and Author n \\
% %         Address line \\ ... \\ Address line}
% % if the names do not fit well on one line use
% %         Author 1 \\ {\bf Author 2} \\ ... \\ {\bf Author n} \\
% % For authors from different institutions:
% % \author{Author 1 \\ Address line \\  ... \\ Address line
% %         \And  ... \And
% %         Author n \\ Address line \\ ... \\ Address line}
% % To start a seperate ``row'' of authors use \AND, as in
% % \author{Author 1 \\ Address line \\  ... \\ Address line
% %         \AND
% %         Author 2 \\ Address line \\ ... \\ Address line \And
% %         Author 3 \\ Address line \\ ... \\ Address line}

% \author{Bo Ai \and Yuchen Wang \and Yugin Tan \and Samson Tan \\
%   Department of Computer Science, National University of Singapore 
% }

% \begin{document}
% \maketitle
% \begin{abstract}
% Authorship attribution is the task of identifying the author of a given text. The key challenge is to find author-specific representations of texts. Most existing approaches hand-engineer features to capture an author's content and style. Due to dataset-specific engineering, these methods are sensitive to different writing topics, writing styles, and other dataset characteristics. In this work, we propose a simple yet effective algorithm that specializes representations without manual design and performs consistently across datasets. The proposed Contra-X fine-tunes pretrained representations and encourages these representations to be distinct for inter-author texts and similar for intra-author texts. This creates a highly distinctive but tight representation subspace for each author. Empirically, we show that Contra-X advances the state-of-the-art on multiple human and machine authorship attribution benchmarks of varying data sizes, writing quality, and author identities. Moreover, we present analyses of these improvements. Our learned representations form highly separable clusters for different authors, and we find that Contra-X trades performance on some authors for improvement in overall accuracy. To the best of our knowledge, we are the first to incorporate contrastive learning into supervised learning for authorship attribution, and our in-depth analysis allows us to better understand the "black-box" learning approach and to identify important questions for future work. \footnote{Code will be made available at \texttt{$<$redacted$>$}}
% \end{abstract}

% \section{Introduction}
% % Structure
% % \begin{itemize}
% %     \item Hook: What is the state of the world/field/community today, what is the significance of this problem and how does it relate to the world? Can tie in to machine generated text detection, how it is a special case of AA.
% %     \item How will the world be changed if we make progress on this problem? (Why should the reader continue reading)?
% %     \item What are the gaps in existing methods? X, Y, Z have done a, b, c, BUT what about d? What did they miss? What are the implications?
% %     \item Some lead-in/background to your method. However, its impact on authorship attribution has not been investigated. 
% %     \item Hence, we contribute/investigate the effect of ..., empirically demonstrate its efficacy on multiple datasets, human and machine-generated texts, while being more sample efficient with the same number of training steps.
% %     \item also propose metrics to analyze how constrastive learning improves authorship attribution performance.
% % \end{itemize}

% \begin{figure}[t]
%     \centering
%     \setlength{\tabcolsep}{2pt} % Default value: 6pt
%     \renewcommand{\arraystretch}{2} % Default value: 1
%     \begin{tabular}{ c c }
%     \includegraphics[width=0.45\columnwidth]{figs/b10_baseline.png} \label{fig:tsne_base} &
%     \includegraphics[width=0.45\columnwidth]{figs/b10_proposed.png} \label{fig:tsne_ours} \\
%     \subfig(a) \bertbase{} & \subfig(b) \bertcl{} \\ 
%     % \includegraphics[width=0.48\textwidth]{figs/matrix_baseline_50_cropped.png} \label{fig:conf_base} &
%     % \includegraphics[width=0.48\textwidth]{figs/matrix_proposed_50_cropped.png}
%     % \label{fig:conf_ours} \\
%     % \subfig(c) \bertbase{} confusion matrix & \subfig(d) \bertcl{} confusion matrix \\ 
%     \end{tabular}
%     \caption{t-SNE visualization of the fine-tuned representations (a: baseline; b: Contra-X). Each color denotes one author in the \blogsmall{} dataset. Our contrastive method effectively creates a tighter representation for each author and increased separation between authors. Best viewed in color. }
%     \label{fig:tsne}
% \end{figure}

% Authorship attribution (AA) is the task of identifying the author of a given text. AA systems are used to identify the authors of anonymous email threats \citep{forensic_1} and historical texts \citep{mendenhall1887characteristic}, to detect plagiarism \citep{forensics_plagiarism}, and more recently to detect machine-generated text \citep{detection_survey}.

% %Authorship attribution (AA) is the task of identifying the author of a given text. AA systems are commonly used to identify the authors of anonymous email threats \citep{forensic_1} and historical texts \citep{mendenhall1887characteristic}, and to detect plagiarism \citep{forensics_plagiarism}. With the rise of neural text generators that can create highly believable fake news \citep{grover}, AA systems are also increasingly used in machine-generated-text detection \citep{detection_survey}. When performed on texts generated by human and machine writers, AA can also act as a \turingtest{} for natural language generation \citep{turing_benchmark, aa_nlg}. 

% Conventional AA methods design features that characterize texts based on their content or writing style \citep{style_aware, syntax_cnn, style_ngram, topic_or_style}. However, this often yields inconsistent performance under varying conditions \citep{topic_or_style}. In contrast, learning features from large corpora of data produces general pre-trained models \citep{bert} that produce superior performance \citep{bertaa}. However, we claim that basic fine-tuning cannot sufficiently capture the key to this task, which is to learn \textbf{\textit{author-specific}} representations. We seek to improve the learning process. 

% Contrastive learning is a technique that pulls similar samples close and pushes dissimilar samples apart in the representation space \citep{simcse}. It has proven useful in tasks that require distinguishing subtle differences \citep{cl_multiview, cl_speech}. This makes it highly suited to learning distinct author subspaces. However, no prior work has investigated its relevance to the AA task. To this end, we seek to understand its impact on the learning of author-specific features under the supervised learning paradigm.

% To achieve this, we integrate \textbf{\uppercase{contra}}stive learning with \textbf{\uppercase{cross}}-entropy finetuning (\textbf{\method{}}) and demonstrate its efficacy via evaluation on multiple human and machine-writer AA datasets. 

% % In addition, we study the performance of our method under different data availability. We find \method{} to consistently improve model performance and yield distinct author subspaces. Finally, we analyze the performance gains vis-\`a-vis a number of AA-specific stylometric features. The analysis helps us understand the strengths of the weaknesses of the approach, which reveals insights for future work. To the best of our knowledge, we are the first to investigate and demonstrate the effectiveness of contrastive learning for authorship attribution.

% % \footnote{\citet{siamese_bert} also investigate contrastive learning but for the task of authorship \textit{verification}, which does not require learning of representations specific to a given author.}

% Our contributions are as follows:
% \begin{itemize}
%     \item We propose and extensively test \method{}. We are one of the first AA works that benchmarks on both human and machine-writer datasets. 
%     \item We advance the state-of-the-art across datasets and show that \method{} is generic to dataset sizes, writing quality, and author identities.
%     \item Beyond empirical performance, we provide in-depth qualitative and quantitative analyses of our results. These help us understand the "black-box" learning approach better and identify important questions for future work.
% \end{itemize}

% % \footnote{\citet{Jafariakinabad, 2021} also investigates contrastive learning, but with a different objective of unifying lexical and syntactic representations of text.}

% \section{Related Work} \label{sec:related_work}
% \paragraph{Authorship attribution.} AA techniques fall under two broad categories: feature-based and learning-based approaches. The former involves hand-crafting features relevant for identifying authors \citep{topic_or_style}; the latter exploits large-scale pretraining to learn text representations. 

% We note that feature-based approaches are investigated in two streams of works. One stream benchmarks on public datasets such as \imdb{} \citep{imdb62} and \blog{} \citep{blog}. The various features proposed include term frequency–inverse document frequency (TF-IDF) \citep{rahgouy2019cross}, letter and digit frequency \citep{topic_or_style}, and character n-grams \citep{char_ngram}. The other stream is the PAN shared task of authorship identification, active before 2019. These methods typically use multiple features such as n-grams \citep{pan1,pan2,pan3,pan5,pan6} in an ensemble. The two streams share similar technical ideas and developments. 

% However, feature-based approaches require dataset-specific engineering \citep{topic_or_style} and their performance does not scale with more data In contrast, learning-based approaches learn representations completely from data. BertAA \citep{bertaa} shows that a simple fine-tuning of pre-trained language models can outperform classical approaches by a clear margin. However, purely cross entropy-based fine-tuning may not exploit the fact that distinctive representations are the key to this task. Thus, we propose to incorporate contrastive learning which enforces distance constraints in the representation space. 

% A concurrent work \citep{han} uses LSTMs that take pre-processed lexical and syntactic information as inputs and trains the model with a contrastive learning objective. Our work is different in that we fine-tune pretrained representations, whose quality scales with data (\secref{sec:experiments_human}), and we adopt a different formulation of the contrastive learning objective. 

% % about PAN
% % PAN 2019 is the latest batch of PAN's authorship attribution task. The cross-domain authorship attribution task at PAN 2019 is an open-set attribution task where an unknown text is to be assigned to a seen candidate author or discarded if no candidate is believed to be the author \citep{pan1}. Architecture wise, all submitted models are non-deep-learning based, employing classifiers including SVM, Logistic Regression (LR), random forest, k-nn, naive Baysed, individually or ensemble, where SVM with LR is found the most effective \citep{pan2, pan3}. One submission of PAN 2018 uses neural network \citep{pan5}, but it is greatly out-performed by the winning submission with an ensemble classfier \citep{pan6}. Feature wise, the majority are using n-grams with TF-IDF weighting. We are not making direct comparison with PAN-related work because the submissions of PAN 2019 have hardware limitations of TIRA \citep{pan4} so the models may be compromised and overly catered to the problem set, and there are more recent and publicly available benchmarks.


% \paragraph{Contrastive learning.} Contrastive learning pulls representations of positive samples closer and pushes those of negative samples apart. Unsupervised contrastive learning has been used for authorship verification \citep{universal}, a binary classification task that determines if two texts come from the same author. Verification is less challenging than attribution, as the latter requires distinguishing many authors of similar writing styles. The difficulty of AA also scales with the number of authors. Contrastive learning is also incorporated with supervised learning for machine translation \citep{supervised_cl}. To the best of our knowledge, we are the first to study the efficacy of integrating contrastive learning with supervised learning on the authorship attribution task. 

% %  speech recognition \citep{cl_speech}, learning sentence embeddings \citep{simcse},

% % The learned representations could be useful for downstream tasks, when the positive and negative sampling scheme matches the task objective.

% % This encourages the learning of highly separable features that can be easily operated on by a downstream classifier. Unsupervised contrastive learning has been used to improve the robustness and transferability of  and to learn sentence embeddings \citep{simcse}. It has also been combined with supervised learning for intent detection \citep{contrastive_pt_ft}, punctuation restoration \citep{supervised_cl_punctuation}, machine translation \citep{supervised_cl}, and dialogue summarization \citep{cl_dialogue}. It is typically useful in tasks that require highly discriminative features. In our work, we integrate supervised learning with contrastive learning. To the best of our knowledge, we are the first to study its efficacy on authorship attribution.

% % We conjecture that this last form of contrastive learning is an effective tool to differentiate authors, and undertake, to our knowledge, the first investigation of the impact and limitations of this approach on our task.

% % As an unsupervised representation learning method, 

% % Contrastive learning can be used as a standalone unsupervised learning technique, or along with a task-specific learning objective.

% %Since authorship attribution requires learning to distinct different authors, we conjecture that contrastive learning is potentially effective. 

% % Contrastive learning is used in was first proposed for facial recognition tasks in computer vision \citep{cl_multiview, cl_visual} to differentiate individuals in the presence of viewpoint changes.

% % t was also used in unsupervised video learning \citep{cl_uncurated_video, cl_unsupervised_video} and knowledge distillation \citep{cl_transfer} to learn or extract more meaningful representations. 

% % However, to our knowledge, there have been no attempts at exploiting contrastive learning for authorship attribution. We conjecture that the nature of this task requires distinction between authors, thus 
% % discriminative features, particularly with many authors or with scarce data. 
% % To this end, we make the first attempt at incorporating contrastive representation learning with unsupervised language pre-training for authorship attribution. 

% %Many works on authorship \textit{verification} (AV), a binary classification task of determining if a pair of samples have the same author, have also used this technique \citep{deep_bayes, siamese_bert, idiolects, compromised_tweet, universal}. 

% % for Authorship \textit{Verification} (AV), a binary classification task of determining if a pair of samples have the same author. As training is done by feeding sample pairs to the network, contrastive loss functions are an intuitive choice as they maximise the output vector difference for negative pairs (i.e., different authors) and minimise it for positive pairs.  all found contrastive learning to work well for AV.

% %\citep{deep_bayes}, \citep{siamese_bert}, \citep{idiolects} and \citep{compromised_tweet} all found contrastive learning to work well for AV. These methods only consider the vector difference between individual pairs of samples. \citep{universal} calculates a single loss across an entire mini-batch of samples, similar to our approach. However, as AA and AV have different corpora and metrics of success, the two sets of results are not directly comparable.

% %However, to the best of our knowledge, there have been no attempts at exploiting contrastive learning for authorship attribution task. We conjecture that the nature of the task requires learning discriminative features and this motivates exploring this technique. To this end, we will make the very first attempt at incorporating contrastive representation learning with unsupervised language pre-training for authorship attribution.

% %\citep{structural} uses a contrastive loss function on a Siamese network architecture with one lexical feature and one structural feature subnetwork. They aimed to minimise the distance between a lexical and a structural representation vector from the same sentence, and maximise it for vectors from different sentences. Our approach differs as we maximise the difference between representation vectors of samples from different authors.

% % \textbf{Neural Language Generation.} 

% \paragraph{Detection of machine generated text.} Modern natural language generation (NLG) models can generate texts indistinguishable from human writings \citep{gpt3, grover}. With the potential for malicious use such as creating fake news \citep{ntg_impact}, detecting machine-generated text is increasingly important. This binary classification task can be extended to a multi-class AA task including both humans and NLG authors. This task can therefore identify not just machine text but also its particular source. Further, \citet{turing_benchmark} proposes that this serves as a \emph{Turing Test} to assess the quality of NLG models. We therefore evaluate our approach on both human corpora and the human-machine dataset \turingbench{}, and show that our approach is generic to author identities and dataset compositions. 

% % Also known as artificial or neural-generated text \textit{detection} \citep{detection_survey, detection_topology}, this is a special type of authorship attribution. 

% % Existing detectors perform inconsistently on texts from different generators \citep{turing_benchmark}. 
% % We investigate how contrastive learning can produce a stable and performant detector as well as its potential limitations. 

% % unlike typical previous work on authorship attribution task that only evaluates the method on human texts, we also present results on 


% \section{Methodology} \label{sec:method}

% \subsection{Problem formulation}
% Authorship attribution is a classification task where the input is some text, $t$, and the target is the author, $a$. Formally, given a corpus $\mathcal{D}$, where each sample is a text-author pair $\langle t, a \rangle$, we aim to learn a predictor, $p$, that maximizes the prediction accuracy. Conventionally, this is achieved by optimizing the cross-entropy loss via mini-batch gradient descent. Assuming we have a mini-batch containing $N$ texts $\{t_i\}_{i=1:N}$ and corresponding authors $\{a_i\}_{i=1:N}$, the loss function is: 
% \begin{equation} \label{ce_loss}
%     \mathcal{L}_{CE} = - \sum_{i} a_i \log(p(t)_{a_i})
% \end{equation}

% % :
% % \begin{equation}
% %     Acc = \E_{\langle{}t, a\rangle{} \in D} \mathds{1}_{argmax(p(t))=a}
% % \end{equation}

% However, we conjecture that $\mathcal{L}_{CE}$ does not adequately reflect the key challenge of the task, which is to learn highly discriminative representations for different authors. Thus, we propose to improve the learning by enforcing distance constraints on the representations. 

% % We conjecture that the key to the authorship attribution task is to learn highly author-specific representations that capture each author's characteristics.

% \subsection{\method{} for Authorship Attribution} \label{sec:cl}
% To distinguish between different authors, we wish the representations to be similar for samples from the same authors, and distinct for samples from different authors. We adopt two specific strategies to achieve this goal: 
% \begin{itemize}[leftmargin=\parindent]\itemsep0em
%     \item Unlike most previous work that hand-crafts features and then learns a predictor $p$ from scratch, we decompose $p$ as $p = \phi \circ h$ where $\phi$ is the pre-trained language model and $h$ is a classifier layer. As shown by BertAA \citep{bertaa}, finetuning the model with cross-entropy outperforms feature engineering approaches. 
%     \item To learn more semantically structured representations, we encourage $\phi$ to capture the idiosyncrasies of each author. This is achieved via a contrastive learning objective. 
% \end{itemize}

% Intuitively, our contrastive objective encourages the model to \textbf{\emph{maximize}} the representational similarity of texts written by the same author, \ie{} positive pairs, and \textbf{\emph{minimize}} the similarity of texts by different authors, \ie{} negative pairs. Formally, we feed each mini-batch of $N$ texts $\{t_i\}_{i=1:N}$ and their authors $\{a_i\}_{i=1:N}$ into a pre-trained language model $\phi$ to obtain a batch of embeddings $\{e_i\}_{i=1:N}$, where $e_i = \phi(t_i)$. Embeddings of two samples by the same author $\langle e_{i}, e_{j} \rangle_{a_i = a_j}$ are a positive pair, and embeddings of two samples by different authors $\langle  e_{i}, e_{j} \rangle_{a_i \neq a_j}$ are a negative pair. We construct a similarity matrix $\mathcal{S}$ in which the entry $(i, j)$ denotes the pairwise similarity between $e_{i}$ and $e_{j}$. Formally, 
% \begin{equation}
%     \mathcal{S}_{i, j}  = \cos(e_i, e_j) = \frac{e_i \cdot e_j}{\|e_i\| \|e_j\|}
% \end{equation}

% To encourage the abovementioned pairwise constraints, we define the contrastive objective as: 
% \begin{align} \label{eqn:cl_term}
%     \mathcal{L}_{CL} = & -\sum_{i} \log(\frac{\sum_{a_i = a_j} \exp(\cos(e_i, e_j)/\tau)}{\sum_{k}  \exp(\cos(e_i, e_k)/\tau)}) \nonumber \\
%     = & -\sum_i \log(\frac{\sum_{a_i = a_j} \exp(\mathcal{S}_{i,j}/\tau)}{\sum_k \exp(\mathcal{S}_{i,k}/\tau))}),
% \end{align}
% where $\tau$ is the temperature which we set to $0.1$. The loss can be viewed as being applied on a softmax distribution to maximize the probability that $e_i$ and $e_j$ come from a positive pair, given $a_i = a_j$. However, it is different from $\mathcal{L}_{CE}$ in that it explicitly enforces pairwise constraints in the representation space $\phi(\cdot)$. During training, we jointly optimize $\mathcal{L}_{CE}$ and $\mathcal{L}_{CL}$:
% \begin{align} \label{eqn:tot_loss}
%     \mathcal{L} = \mathcal{L}_{CE} + \mathcal{L}_{CL},
% \end{align}
% This joint optimization, \method{}, improves upon $\mathcal{L}_{CE}$ by mining richer knowledge in the training data via encouraging meaningful pairwise relations in the representation space $\phi(\cdot)$. We conjecture that the model learns discriminative features in alignment with the classification objective. This will be empirically examined (\secref{sec:experiments_human} and \secref{sect:results_nlg}) and qualitatively analyzed (\secref{sect:discuss_visualize}). 

% % Compared to traditional methods, our method encourages the model to discover discriminative representations for different authors without human features. We will show that our method yields consistent performance improvements over the baseline in a variety of datasets, \ie human and machine writing corpora. 

% \subsection{Implementation Details}

% % \begin{table*}[t]
% % \centering
% % \begin{tabular}{c c c c c}
% %   \toprule
% %   Model & \blogsmall{} & \blogbig{} & \imdb{} & \enron{} \\
% %   \midrule
% %   Token SVM \citep{imdb62} & - & - & 92.5 & - \\
% %   Char-CNN \citep{char_cnn} & 61.2 & 49.4 & 91.7 & - \\
% %   Continuous N-gram \citep{conti_ngram} & 61.3 & 52.8 & 95.1 & - \\
% %   N-gram CNN \citep{ngrams_cnn} & 63.7 & 53.1 & 95.2 & - \\
% %   Syntax CNN \citep{syntax_cnn} & 64.1 & 56.7 & 96.2 & - \\
% %   BertAA \citep{bertaa} & 65.4 & 59.7 & 93.0 & 97.1 \\ 
% %   \midrule
% %   \bertbase{} \textit{(our baseline)} & 60.4 & 55.2 & 97.2 & 97.6 \\
% %   \bertcl{} & 66.3 (5.9\textcolor{black}{$\uparrow$}) & 62.0 (6.8\textcolor{black}{$\uparrow$}) & 97.9 (0.7\textcolor{black}{$\uparrow$}) & 97.6 \\
% %   \debertabase{} \textit{(our baseline)} & 69.1 & 64.7 & 98.1 & 97.9 \\
% %   \debertacl{} & \textbf{69.7 (0.6\textcolor{black}{$\uparrow$})} & \textbf{68.4 (3.7\textcolor{black}{$\uparrow$})} & \textbf{98.2 (0.1\textcolor{black}{$\uparrow$})} & \textbf{98.0 (0.1\textcolor{black}{$\uparrow$})} \\
% %   \bottomrule
% % \end{tabular}
% % \caption{Results on human AA datasets (accuracy). Results in top section are from their respective papers. The best model for each dataset is \textbf{bolded}. Improvements over the baselines are indicated in parentheses. }
% % \label{table:sota}
% % \end{table*}

% % \begin{table*}[t]
% % \centering
% % \begin{tabular}{c c c c}
% %   \toprule
% %   \textbf{Model} & \textbf{\blogsmall{}} & \textbf{\blogbig{}} & \textbf{\imdb{}} \\
% %   \midrule
% %   Token SVM \citep{imdb62} & - & - & 92.5 \\
% %   Char-CNN \citep{char_cnn} & 61.2 & 49.4 & 91.7 \\
% %   Continuous N-gram \citep{conti_ngram} & 61.3 & 52.8 & 95.1 \\
% %   N-gram CNN \citep{ngrams_cnn} & 63.7 & 53.1 & 95.2  \\
% %   Syntax CNN \citep{syntax_cnn} & 64.1 & 56.7 & 96.2 \\
% %   BertAA \citep{bertaa} & 65.4 & 59.7 & 93.0  \\ 
% %   \han{} \citep{han} & \textbf{73.5} & 61.7 & - \\
% %   \midrule
% %   \bertbase{} \textit{(our baseline)} & 60.4 & 55.2 & 97.2  \\
% %   \bertcl{} & 66.3 (5.9\textcolor{black}{$\uparrow$}) & 62.0 (6.8\textcolor{black}{$\uparrow$}) & 97.9 (0.7\textcolor{black}{$\uparrow$}) \\
% %   \debertabase{} \textit{(our baseline)} & 68.1 & 64.7 & 97.8 \\
% %   \debertacl{} & 69.8 (1.7\textcolor{black}{$\uparrow$}) & \textbf{68.4 (3.7\textcolor{black}{$\uparrow$})} & \textbf{98.3 (0.5\textcolor{black}{$\uparrow$})}  \\
% %   \bottomrule
% % \end{tabular}
% % \caption{Results on human AA datasets, measured in accuracy. Following previous work in this table, we specify a precision of 1 decimal place. Results in the top section are from their respective papers, except for \citet{conti_ngram} and \citet{ngrams_cnn} which were reported by \citet{syntax_cnn}. Improvements over the baselines are indicated in parentheses. We report the average accuracy of ten-fold cross validation. The best model for each dataset is \textbf{bolded}.}
% % \label{table:sota}
% % \end{table*}

% \begin{table*}[t]
% \centering
% \begin{tabular}{c c c c}
%   \toprule
%   \textbf{Model} & \textbf{\blogsmall{}} & \textbf{\blogbig{}} & \textbf{\imdb{}} \\
%   \midrule
%   Token SVM \citep{imdb62} & - & - & 92.5 \\
%   Char-CNN \citep{char_cnn} & 61.2 & 49.4 & 91.7 \\
%   Continuous N-gram \citep{conti_ngram} & 61.3 & 52.8 & 95.1 \\
%   N-gram CNN \citep{ngrams_cnn} & 63.7 & 53.1 & 95.2  \\
%   Syntax CNN \citep{syntax_cnn} & 64.1 & 56.7 & 96.2 \\
%   BertAA \citep{bertaa} & 65.4 & 59.7 & 93.0  \\ 
%   \han{} \citep{han} & \textbf{73.5} & 61.7 & - \\
%   \midrule
%   \bertbase{} \textit{(our baseline)} & 60.4 ($\pm$0.6) & 55.2 ($\pm$0.7) & 97.2 ($\pm$0.1) \\
%   \bertcl{} & 66.3 ($\pm$0.7) & 62.0 ($\pm$0.5) & 97.9 ($\pm$0.2) \\
%   \debertabase{} \textit{(our baseline)} & 68.1 ($\pm$0.7) & 64.7 ($\pm$0.8) & 97.8 ($\pm$0.2) \\
%   \debertacl{} & 69.8 ($\pm$0.5) & \textbf{68.4 ($\pm$0.7)} & \textbf{98.3 ($\pm$0.2)}  \\
%   \bottomrule
% \end{tabular}
% \caption{Test accuracy on human AA datasets. We report the mean values from 10-fold cross validation, and standard deviations are indicated in parentheses. Following previous work, we specify a precision of 1 decimal place. The improvements of \method{} over baselines are positive with statistical significance $p < 10^{-5}$. Results in the top section are from their respective papers, except for \citet{conti_ngram} and \citet{ngrams_cnn} which were reported by \citet{syntax_cnn}. The best model for each dataset is \textbf{bolded}.}
% \label{table:sota}
% \end{table*}

% We implement $\phi$ with two pre-trained transformer encoders,\footnote{We omit other notable architectures such as convolutional or recurring neural networks and focus solely on pre-trained models as 1. we theorize Contra-X to be effective at optimizing learned language representations, which are only present in pre-trained models, and 2. pre-trained models offer state-of-the-art performance in many benchmarks, and are thus the best candidate for further research.} BERT \citep{bert} and DeBERTa \citep{deberta}.\footnote{BERT is the pioneering transformer architecture commonly used for benchmarks, and DeBERTa is one of the best-performing recent variants.}  We use the \texttt{bert-base-cased} and \texttt{deberta-base} checkpoints from the \texttt{transformers} library \citep{huggingface}. For all datasets, the input length is set to $256$ and the embedding length per token to $768$. The transformer generates embeddings which are then passed to the classifier $h$. 

% % We concatenate the token embeddings to obtain a sentence embedding of length $196608$. The embedding is then passed to the classifier $h$. 

% We implement $h$ as a 2-layer Multi-Layer Perceptron (MLP) with a dropout of $0.35$. As described in \secref{sec:cl}, the final model $p$ is a composition of the pre-trained language model and the MLP classifier, \ie{} $p = \phi \circ h$.

% In all experiments, we use the AdamW optimizer \citep{adamw} with an initial learning rate of $2e-5$ and a cosine learning rate schedule \citep{sgdr}. We train for $8$ epochs with a batch size of 24. Training takes 2-12 hours depending on the dataset size with $4~\times$ RTX2080Ti. 

% % No model- or dataset-specific tuning was done for fair comparison and to show the robustness of the approach. 

% \section{Human Authorship Attribution} \label{sec:experiments_human}

% We first investigate the impact of contrastive learning on models for human authorship attribution.

% \subsection{Experiment setup} 
% \label{sec:human_exp_setup}

% \paragraph{Models.} We experiment with four different models: two baselines \bertbase{} and \debertabase{}, fine-tuned with cross-entropy, and their \method{} versions, \bertcl{} and \debertacl{}. These baselines allow us to isolate the effect of the proposed contrastive learning objective $\mathcal{L}_{CL}$.

% %We run each model on three popular authorship attribution corpora, which represent potential real-world use cases of identifying human authors.


% %This is the standard task studied in most of the previous works. 

% % We first conduct authorship attribution experiments on human-written materials. The experiment results show the effectiveness of 1) the fine-tuned pre-trained models and 2) the contrastive learning technique.  

% % \subsection{Experimental Setup}

% \paragraph{Datasets.} Following prior work \citep{char_cnn,syntax_cnn,bertaa}, we use the Blog \citep{blog} and IMDb \citep{imdb62} corpora for evaluation. For Blog, we take the top 10 and 50 authors with the most entries to form the \blogsmall{} and \blogbig{} datasets respectively \citep{syntax_cnn,bertaa}. For IMDb, we take a standard subset of 62 authors \citep{imdb62} (\imdb). More details are in \appendixref{sect:statistics}.

% \paragraph{Evaluation.} Following previous state-of-the-art authorship attribution tasks \citep{imdb62, char_cnn, conti_ngram}, we run experiments with ten-fold cross-validation. 

% % For easy comparison, we also present results on the 8:2 train/test splits used by \citet{bertaa} in \appendixref{sect:result82}. We do not observe any significant differences.

% % Following standard evaluation protocol, we divide each dataset into train/validation/test splits with an 8:1:1 ratio, and report the test split results here. Hyperparameter tuning, if any, is performed on the validation set. 
% % We adopt the accepted machine learning best practice for evaluating our method. Instead of using 8:2 train/test splits as in \citet{bertaa}, we divide the dataset into train/validation/test splits with ratio 8:1:1. However, results on the 8:2 splits are also available in \appendixref{sect:result82}. The two sets of results differ only slightly.

% % \subsection{Results}

% % Full results are shown in \tabref{table:sota}.\footnote{The baseline results are reported by their respective papers, except for Continuous N-Gram \citep{conti_ngram} and N-gram CNN \citep{ngrams_cnn} which are reproduced and reported by \citet{syntax_cnn}.} 

% \subsection{Results} 
% From \tabref{table:sota}, we observe that the inclusion of contrastive learning improves baseline performance across the board, allowing us to beat all previous states-of-the-art on all human AA datasets except for HAN (which is a contemporaneous work). We believe this is because HAN extracts hand-crafted lexical and syntactic features for classification, which reduces the data required to learn a decent classifier. However, these hand-crafted features may be restrictive if more data is available or the task is harder; thus our method outperforms HAN on \blogbig{}.

% In terms of improvements brought by contrastive training, the largest gains appear in \blogsmall{} and \blogbig{} where there is substantial room for improvement. In contrast, the performance gains on \imdb{} are marginal due to diminishing returns, with the baseline models already achieving close to 100\% accuracy. These results suggest that this application of contrastive learning is most useful when the baseline performance is not approaching an asymptotic maximum.

% % \textbf{\blogsmall{} and  \blogbig{}.}  Our approach with \bertcl{} improves the performance of \bertbase{} by 5.9\% and 6.8\% respectively. As \debertabase{} already achieves high performance on both datasets, the further improvements from \debertacl{} are relatively smaller. It is worth noting that \debertabase{} with simple finetuning already outperforms all previous results, showing the effectiveness of using learned language representations. \debertacl{} makes further gains on this baseline, showing the effect of the contrastive learning objective. 

% % \textbf{\imdb{} and \enron{}.} Existing results on \imdb{} and \enron{} are already close to 100\%, making the margin for improvement small. On \imdb{}, both \bertcl{} and \debertacl{} make marginal gains on their non-contrastive counterparts. On \enron{}, \debertacl{} improves on \debertabase{} slightly.

% % Our results show that learned language representations are effective for authorship attribution task, while contrastive learning further improves the performance. This empirically verifies the effectiveness of our strategies in \secref{sec:cl}.


% \section{Synthetic Text Authorship Attribution} \label{sect:results_nlg}

% We investigate our proposed models on AA datasets with neural-generated text. This is to show how our method performs consistently across different dataset qualities and writers. Performing AA on human and machine authors together also reflects the increased importance of identifying machine-generated text sources. 

% % Thirdly, this potentially reveals information about how differently machines write compared to humans.

% % In this section, we show that our method is general and can achieve state-of-the-art results on machine datasets. 

% % our proposed models and loss function are proved useful in learning generated texts as well as differentiating human and machine writers. 

% \subsection{Experimental Setup} \label{sect:results_nlg_setup}

% \paragraph{Models.} We test the same four models from \secref{sec:experiments_human}: \bertbase{}, \bertcl{}, \debertabase{}, and \debertacl{}.

% \paragraph{Dataset.} We use the \turingbench{} dataset \citep{turing_benchmark}. This corpus contains 200,000 news articles from 20 authors (one human and 19 neural language generators). The task of authorship attribution here implicitly encompasses the easier binary classification task of machine text detection. Dataset statistics are available in \appendixref{sect:statistics}. 

% % This corpus contains 200,000 human-written or machine-generated texts from 20 sources, consisting of 1 human and 19 neural language generators. The 10,000 human-written texts are first collected from news articles from medias such as CNN, then 19 neural language models generate the rest 190,000 texts given the titles.  The motivation of the benchmark is that it resembles the \turingtest{} for neural language generation methods. 

% %Thus, the topical difference between samples is smaller than previous humans datasets.

% \paragraph{Evaluation.} We use the 7:1:2 train/validation/test splits provided by \citet{turing_benchmark} and report the results on the test set. 

% \subsection{Results}

%  \tabref{table:sota_nlg} shows the results of the synthetic AA benchmark. Contrastive learning provides a clear accuracy improvement over the baseline models, in particular allowing \debertacl{} to set a new state-of-the-art. This suggests that our approach generalizes to different writers and corpus compositions without dataset-specific engineering. 
 
% %  \footnote{For consistency, we report results to 2 decimal places. For full results for other metrics, \ie{}  precision, recall, and F1-score, see \appendixref{sec:full_turing_results}.}
 
% %  Our proposed model \debertacl{} outperformed all previous results, and further improves the performance of \debertabase{} by 0.53\%. Note that our \bertbase{} did not reach the previous reported result by BERT, which indicates that our method may not have reached its full performance given we did not perform hyperparameter tuning.

% %Furthermore, it reveals that our approach may be applicable to relevant tasks such as fake review detection \citep{fake_review}.

% \begin{table}[t]
% \centering
% \begin{tabular}{c c}
%   \toprule
%   \textbf{Model} & \textbf{\turingbench} \\
%   \midrule
%   Random Forest & 61.47 \\
%   SVM (3-grams) & 72.99 \\
%   WriteprintsRFC & 49.43 \\
%   OpenAI Detector & 78.73 \\
% %   \footnote{\url{https://huggingface.co/roberta-base-openai-detector}}
%   Syntax CNN & 66.13 \\
%   N-gram CNN & 69.14 \\
%   N-gram LSTM-LSTM & 68.98 \\
%   BertAA  & 78.12 \\ 
%   BERT & 80.78 \\
%   RoBERTa & 81.73 \\
%   \midrule
%   \bertbase{} \textit{(our baseline)} & 79.16 \\
%   \bertcl{} & 80.59 (1.43\textcolor{black}{$\uparrow$})\\
%   \debertabase{} \textit{(our baseline)}  & 81.80 \\
%   \textbf{\debertacl{}} & \textbf{82.53 (0.73\textcolor{black}{$\uparrow$})}\\
%   \bottomrule
% \end{tabular}
% \caption{Results on human and machine authorship attribution (accuracy). Results in top section are from the \turingbench\ paper. Improvements over the baselines are indicated in parentheses. Best model is \textbf{bolded}.}
% \label{table:sota_nlg}
% \end{table}

% \section{Discussion} \label{sec:discussion}
% In this section, we study the following questions:
% \begin{itemize}[leftmargin=\parindent]\itemsep0em
%     \item How does data availability affect performance with and without contrastive learning?
%     % \item How does availability of data affect the performance of fine-tuning? How can our approach influence the performance?
%     \item How does contrastive learning qualitatively affect the representations learned?%Why does our proposed approach work? What representations does it learn?
%     \item When does \method\ succeed and fail? 
% \end{itemize}

% % We will present corresponding analyzes in the following subsections. 

% \begin{table}[t]
% \centering
% \begin{tabular}{p{0.18\linewidth} | p{0.75\linewidth}}
%   \toprule
%   \textbf{Author} & \textbf{Sample} \\
%   \midrule
%   5 & Dude...we shoulda taken the trip to that doctor...don't say I didn't tell you so.  HEY, good news! Cary McNamara screwed with the votes somehow so they're re-doing the whole election by paper ballots! \\
%   6 & OMG i JUST realized....alot of people have posted here....now we just have to drag Will and Zabeth from where ever they are \\
%   7 & Well, I don't mean to be a show-off, but it seems I'm one of those few who are actually enjoying school. I guess it's going to change after I take a couple of those eighty-percent exams. \\
%   \bottomrule
% \end{tabular}
% \caption{Samples from overlapping (authors 5 \& 6) and distinct (author 7) clusters.}
% \label{table:blog_samples}
% \end{table}

% \subsection{Performance vs. Dataset Size}

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=1.0\columnwidth]{figs/shrinked.png}
%     \caption{Comparison of performance between \bertbase{} and \bertcl{} under different data regimes. }
%     \label{fig:small_dataset}
% \end{figure}

% % The availability of data has been a crucial concern for learning-based approaches. Thus, it is worthwhile to exam the impact of reducing the dataset size.

% Due to the often-adversarial nature of real-world AA problems, availability of appropriate data is a concern. Therefore, it is important to examine the impact of data availability on potential AA systems. To do this, we construct 4 subsets of the \blogsmall{}, \blogbig{}, and \turingbench{} datasets with stratified sampling by author. Each subset is 25\%, 50\%, 75\%, and 100\% the size of the original dataset. We use the same setup as in \secref{sec:human_exp_setup} to train \bertbase{} and \bertcl{} on each subset. 

% % For example, a plagiarism-detection model is unlikely to have a large number of sample texts per student to draw from.

% % Therefore, it is worth examining the impact of  To do this, we take stratified samples of the \blogsmall{} dataset based on authors. We shrink the dataset by 7 ratios, evenly spaced between $12.5\%$ and $87.5\%$ inclusive. Then use the same setup to train \bertbase{} and \bertcl{} on each subsampled set. The results are presented in \figref{fig:small_dataset}.

% \figref{fig:small_dataset} plots accuracy against dataset size to illustrate performance with different amounts of data. On \blogsmall{}, \bertcl{} maintains a surprisingly consistent level of accuracy while \bertbase{} suffers significant degradation in performance as data decreases. On \blogbig{}, \bertcl{} shows more substantial performance gains compared to \bertbase{} as the dataset size increases. We hypothesize that the latter task is intrinsically harder due to the larger number of authors, requiring a larger amount of data to learn well. Even so, \method{} improves the performance of both BERT and DeBERTa by 6.8\% and 3.7\% respectively on the full dataset. On \turingbench{}, the difference in accuracy is less obvious, although \bertcl{} maintains an advantage. A possible explanation is that even the smaller subsets are sufficiently large for \bertbase{} to perform well. 

% From the above, we observe consistent improvements across different data regimes. This is possibly because the contrastive objective explicitly encourages the model to focus on inter-author differences as opposed to irrelevant features. 

% % This can be seen as an regularization effect. However, note that such regularization-like effect does not restrict the model performance as data becomes abundant. This is a potentially important characteristic of \method{}: it is both efficient and scalable. 

% % the baseline performance consistently across dataset sizes and data requirments, \ie{} being efficient and scalable.

% % retain a high level of accuracy for authorship attribution and possibly other general classification tasks when large amounts of training data are not available.
% % it learns not only the representative features of each class but also the difference between authors. In contrast, as the \bertbase{} fine-tuning approach relies on the expressiveness of the deep neural network to learn task-specific representations, it is prone to overfitting. Furthermore, the additional constraints set by the contrastive objective (\eqnref{eqn:tot_loss}) prevent the model from overfitting, providing a regularization effect. 

% % We note the following observations. First, as the \bertbase{} finetuning approach relies on the expressiveness of the deep neural network to learn task-specific representations, it is prone to overfitting. This causes degradation in the test performance as dataset size becomes smaller. Secondly, while the baseline \bertbase{} performance drops significantly with less data, our proposed model maintains a decent level of accuracy. Note that when we only use 12.5\% of the data to train the model, our proposed method can improve the accuracy by 9.2\%. 

% % This illustrates that our proposed approach has a regularization-like effect on the learning and alleviates overfitting when the data is scarce, which is a promising property in many practical applications.

% % We consider this advantage a positive effect of contrastive learning. The understanding is that the model not only learns the representative features of each class but also learns the differences between authors, \ie{} their distinctive writing styles. The additional constraints set by the contrastive objective \eqnref{eqn:tot_loss} enforces additional constraints and prevent the model from overfitting. In other words, it has a regularization effect and improves the sample efficiency of learning. 

% % Our approach of contrastive learning is shown to maintain robust performance in cases of data scarcity, from testings on Blog10 with shrinked dataset. Specifically, we reduce the number of samples per author to its $75\%$, $50\%$, $25\%$, and so on, and compare the results with the baseline approach without contrastive learning. As reflected by Figure \ref{fig:small_dataset}, while the baseline model's performance drops severely with less data, our proposed model maintains a decent accuracy. This illustrates that the proposed method has relatively low sensitivity to the size of the dataset, which is a promising property in practical applications when not many samples are available. We consider this advantage a positive effect of contrastive learning where the model not only learns the representative features of each class but also pays attention to the difference between different authors (i.e. authors' distinctive writing styles). As a result, there is a higher probability that the model can capture unique patterns for each class within limited samples, compared to baseline approach where sufficient amount of data is a necessity. %explain the reason with reference / clustering images

% \begin{table*}[t]
%     \centering
%     \begin{tabular}{c | c c c c | c c}
%       \toprule
%       & \multicolumn{4}{c|}{\textbf{Feature Type}} & \multicolumn{2}{c}{\textbf{Accuracy Improvement}} \\
%       Dataset & Content & Style & Hybrid & Topic & \bertbase\ & \debertabase\ \\
%       \midrule
%       \blogsmall{} & 0.82472 & \textbf{0.33766} & \textbf{0.59218} & 0.85465 & 5.9 & 1.7 \\
%       \blogbig{} & 1.0000 & 1.0000 & 1.0000 & \textbf{0.81145} & 6.8 & 3.7\\
%       \turingbench{} & \textbf{0.60842} & 0.56926 & 0.91988 & 1.0000 & 1.43 & 0.73 \\
    
%     %   Content & 0.63299 & 0.76752 & \textbf{0.46698}\\
%     %   Style & \textbf{0.000156} & 0.000462 & 0.000263\\
%     %   Hybrid & \textbf{0.03363} & 0.05679 & 0.05224 \\
%     %   Topic & 0.23303 & \textbf{0.22125} & 0.27266 \\
%     %   \midrule
%     %   \bertbase{} & 5.9 & \textbf{6.8} & 1.13 \\ 
%     %   \debertabase{} & 0.6 & \textbf{3.7} & 0.53 \\ 
%       \bottomrule
%     \end{tabular}
%     \caption{Inter-author difference on different feature metrics (improvements from each contrastive model listed for reference). The smaller the value, the higher the similarity measured by that feature. For consistency, each column is linearly scaled such that the maximum is 1. The smallest value for each feature is \textbf{bolded}.}
%     \label{table:dataset_similarity_test}
% \end{table*}

% \subsection{Qualitative Representational Differences} \label{sect:discuss_visualize}

% % \begin{table*}[t!]
% % \centering
% % \caption{Inter-Author Similarity of Different Datasets - Lower is more similar}
% % \label{table:dataset_similarity}
% % \begin{tabular}{c c c c c c}
% %   \toprule
% %   Dataset & \blogsmall{} & \blogbig{} & \imdb{} & \enron{} & \turingbench{} \\
% %   \midrule
% %   Content & 0.63299 & 0.76752 & 0.62821 & 0.70303 & \textbf{0.46698}\\
% %   Style & \textbf{0.000156} & 0.000462 & 0.000336 & 0.001062 & 0.000263\\
% %   Hybrid & 0.03363 & 0.05679 & \textbf{0.02057} & 0.16628 & 0.05224 \\
% %   Topic & 0.23303 & 0.22125 & \textbf{0.10556} & 0.43489 & 0.27266\\
% %   \bottomrule
% % %   \caption{Lower values represent greater similarity.}
% % \end{tabular}
% % \end{table*}

% % Extensive empirical results have been reported, but a qualitative analysis of what the model learns is preferable. Thus, in this subsection, we inspect the learned representations to qualitatively explain why the proposed method could be effective. 

% % Specifically, we project representations $\phi(\cdot) \in \mathbb{R}^{196608}$ generated on test-set samples of \blogbig{} to $\mathbb{R}^2$ with t-SNE \citep{tsne}. We present the comparison between \bertbase{} and \bertcl{} in \figref{fig:confusion}.

% % From \figref{fig:confusion}, it is clear our method produces representations that easily distinguish between different authors, while standard fine-tuning does not.
% % %\bertbase{} produces representations spread out in the visualization space, whereas \bertcl{} produces highly separated and concentrated clusters.
% % Note that each cluster corresponds to one author class as labelled out. The observation is attributed to the loss term $\mathcal{L}_{CL}$ that encourages the representation to be similar for intra-author samples, \ie{} smaller spread for the clusters, and to be different for inter-author samples, \ie{} large distance between different clusters. This qualitatively showcases the effectiveness of our approach. 

% Next, we visualize the learned representations to understand the qualitative effect of the contrastive learning objective. We embed the test samples from the \blogsmall{} dataset and visualize the result using t-SNE \citep{tsne}. 

% Qualitatively, it is clear that \bertcl{} produces more distinct and tighter clusters compared to \bertbase{} (\figref{fig:tsne}). Since $\mathcal{L}_{CL}$ is the only independent variable in the experiment, differences in representation can be attributed to the contrastive objective. The improvement is expected, because the objective $\mathcal{L}_{CL}$ explicitly encourages the representation to be similar for intra-author samples (\ie{} tight clusters) and different for inter-author samples (\ie{} larger distance between clusters). This supports our conjecture in \secref{sec:cl}. 

% % Qualitatively, this suggests that the contrastive loss objective is working as intended.

% % From the confusion matrices, we can also observe performance improvements corresponding to changes in the visualization. Compared to \figref{fig:confusion}\subfig(c), the cells along the diagonal line in \figref{fig:confusion}\subfig(d) generally have a darker color, \ie{} higher class-level accuracy, and there are fewer dark points among the rest of the cells, \ie{} lower false positive and false negative rate. Overall, \bertcl{} has a $6.6\%$ improvement in absolute accuracy over \bertbase{}. We conjecture that the separation and concentration effects of $\mathcal{L}_{CL}$ contribute to this performance improvement. 

% However, we observe that some clusters still overlap and are inseparable by t-SNE. This suggests that the model still faces some difficulty in distinguishing between specific authors. \tabref{table:blog_samples} shows some samples from \blogsmall{}. Manual inspection suggests that that overlapping authors (5 and 6) appear to write very similarly (in terms of \eg{} tone of voice), where even a human might struggle to differentiate the two. Meanwhile, author 7, with a distinct and non-overlapping cluster, writes markedly differently. This indicates the model learns meaningful representations consistent with human understanding of language.

% \subsection{When Does \method{} Succeed and Fail?}

% Finally, we examine the conditions under which \method{} is more or less effective. This analysis would enable us to understand our approach beyond the empirical results. 

% % \begin{table}[t]
% %     \centering
% %     \setlength{\tabcolsep}{2pt}
% %     \caption{Inter-author difference (lower is more similar) and improvements from contrastive models on different datasets}
    

% % \begin{table}[t]
% %     \centering
% %     \setlength{\tabcolsep}{2pt}
% %     \caption{Inter-author similarity of different datasets - Lower is more similar}
% %     \label{table:dataset_similarity}
% %     \begin{tabular}{c c c c c c}
% %       \toprule
% %       Dataset & \blogsmall{} & \blogbig{} & \turingbench{} \\
% %       \midrule
% %       Content & 0.63299 & 0.76752 & \textbf{0.46698}\\
% %       Style & \textbf{0.000156} & 0.000462 & 0.000263\\
% %       Hybrid & \textbf{0.03363} & 0.05679 & 0.05224 \\
% %       Topic & 0.23303 & \textbf{0.22125} & 0.27266 \\
% %       \bottomrule
% %     %   \multicolumn{4}{c}{Contrastive Learning Improvement (\%) (ref.)}\\
% %       \bertbase{} & 5.9 & \textbf{6.8} & 1.13 \\ 
% %       \debertabase{} & 0.6 & \textbf{3.7} & 0.53 \\ 
% %       \bottomrule
% %     \end{tabular}
% % \end{table}

% % \begin{table}[t]
% % \begin{tabular}{c c c c c c}
% %       \toprule
% %       Model & \blogsmall{} & \blogbig{} & \turingbench{} \\
% %     %   \multicolumn{4}{c}{Contrastive Learning Improvement (\%) (ref.)}\\
% %       \bertbase{} & 5.9 & \textbf{6.8} & 1.13 \\ 
% %       \debertabase{} & 0.6 & \textbf{3.7} & 0.53 \\ 
% %       \bottomrule
% %     \end{tabular}
% % \end{table}

% %We now seek to study the conditions in which contrastive learning does or does not work. We note that there are many confounders such as the mean and variance in the sentence lengths, dataset size, number of authors, dataset balancedness,  and some other unknown or uncontrollable effects.  Nevertheless, we seek to find some correlations between the model performance and the linguistic characteristics of datasets. We hope the insights to be valuable for improving the contrastive learning method in future, or to understand the authorship attribution task in general. 

% \textbf{Class imbalance.} In any classification task, classes with fewer training samples can be more difficult for models to predict correctly. We find that the class-level improvement of \method{} has no correlation to the number of samples per class in the dataset.\footnote{Due to space contraints, detailed statistics are presented in \appendixref{sec:imbalance}} This suggests that \method{} can be applied on imbalanced datasets without compromising performance.

% \textbf{Linguistic characteristics.} Diversity of stylometric features across a dataset can affect a model's ability to differentiate authors. We follow \citet{topic_or_style} and extract $4$ features: topic, style, content, and hybrid features. Detailed descriptions for each feature are in \appendixref{sec:similarity_metrics}. For this set of features, $\mathcal{F}$, the corresponding feature extractors are $\phi_f$, $f \in \mathcal{F}$. We can then represent each author, $A_i$, with a feature. Given an author $A_i$ with \textit{N} documents $\{t_i\}_{i=1:N}$, we define the representation of $A_i$ to be the mean of the vector representations of the $N$ documents: 

% % \begin{equation} \label{avg_auth_feat}
% %     \bar{F}_{feat}^{\mathcal{A}} = \frac{1}{n} \sum_{i}^{n} {F}_{feat}(t_i)
% % \end{equation} 

% \begin{equation} \label{avg_auth_feat}
%     v_{A_i}^{f} = \frac{1}{N} \sum_{i=1}^N \phi_f (t_i). 
% \end{equation} 

% We analyze the relation between model performance and dataset characteristics below. We exclude \imdb{} from this analysis since the maximum margin for improvement on the dataset is too small ($<3\%$). Performing analysis on these datasets may introduce confounding factors.  

% %In this section, we inspect the correlation between model performance and dataset characteristics to find out when our method works and what its limitations are. Note that the there could be many confounders, such as input sentence, dataset size, the number of authors, and some unmodeled effects, but we seek to identify the potentially relavant factors and study its correlation with model performance. We follow \citet{topic_or_style} to analyze the dataset characteristics. Specifically, we extract 4 types of features from the dataset: topic, style, content, and hybrid features. The description for each feature is in \appendixref{sec:similarity_metrics}.  For each document in the corpus, we extract one feature vector $F_{feat}$ for each of the four features. Given an author $\mathcal{A}$ with \textit{n} documents $\{t_i\}_{i=1:n}$, the overall representation for a certain feature for $\mathcal{A}$ is the mean of the vectors for all \textit{n} documents:

% % \begin{equation} \label{avg_auth_feat}
% %     \bar{F}_{feat}^{\mathcal{A}} = \frac{1}{n} \sum_{i}^{n} {F}_{feat}(t_i)
% % \end{equation} 

% % where $feat \in \{content, hybrid, style, topic\}$. We will further make use of the feature in the following analysis. Note that the baseline performance on \imdb{} and \enron{} datasets are close to 100\% and this implies small margin for improvement. To avoid confounders, we will focus our analysis on the rest 3 datasets. 

% % Finally, we look into the circumstances under which contrastive learning is effective. Following \citet{topic_or_style}, we define four metrics for quantifying the characteristics of an author: topic, style, content, and hybrid features. See Appendix \ref{sec:similarity_metrics} for details on each feature class.

% \paragraph{Dataset-level analysis.} %Our first objective is to look for pattern at the dataset level. To do this, we need to study the correlation between the features from a dataset and their respective margins of improvement from contrastive learning. 
% We quantify the difficulty of distinguishing any two authors in each dataset and compare them against performance improvements. We define the inter-author dissimilarity of a dataset $\mathcal{D}$ in a feature space $f \in \mathcal{F}$ to be the mean pairwise difference across all author pairs $\langle A_i, A_j \rangle$ measured by the feature $f$:

% % \begin{equation} \label{avg_dataset_feat}
% %     \bar{F}_{feat}^{\textit{D}} = \frac{1}{n^{2}} \sum\limits_{\mathcal{A}_i \\ \in D}\sum\limits_{\mathcal{A}_j \in D} Dist(\bar{F}_{feat}^{\mathcal{A}_i}, \\ \bar{F}_{feat}^{\mathcal{A}_j})
% % \end{equation} 

% \begin{equation} \label{avg_dataset_feat}
%     v_{\mathcal{D}}^f = \frac{1}{|A|^2}  \sum_{A_i, A_j \in \mathcal{D}} d(v_{A_i}^f, v_{A_j}^f), 
% \end{equation} 

% where $d$ is a distance metric for a pair of vectors:
% % \vspace{-0.05in}
% \begin{equation} 
% d(v_{A_i}^f, v_{A_j}^f) = 
%     \begin{cases}
%     JSD(v_{A_i}^f, v_{A_j}^f) & \text{if} f = topic \\
%     1 - \cos(v_{A_i}^f, v_{A_j}^f) & \text{otherwise}.
%     \end{cases}
% \end{equation} 

% where JSD is the Jenson-Shannon Divergence \citep{jsd} and $\cos{}$ is the cosine similarity. Lower values indicate a greater average difficulty in distinguishing the authors in a dataset in the corresponding feature space. %The values for the 3 datasets are presented in \tabref{table:dataset_similarity_test}. 

% % where $d$ is a distance metric for a pair of vectors. In our case, it is Jenson-Shannon Divergence (JSD) \citep{jsd} for $f = topic$, or (1 - cosine similarity) otherwise. 

% From \tabref{table:dataset_similarity_test}, we observe that \blogbig{} has both the highest degree of topical similarity and largest improvement from contrastive learning, while \turingbench{} has the least topical similarity and also the least improvement. This suggests that contrastive learning may be more useful when authors in a dataset write about highly similar topics. On the other hand, the opposite is true for content similarity: \turingbench{} has the highest content similarity and yet the least improvement.

% % This may be explained by how content similarity as we define it measures word \textit{n}-gram frequencies, while our contrastive objective (\eqnref{eqn:cl_term}) is applied to the sentence embeddings $\phi(\cdot)$. This does not lead to significant information gain if the sentences contain similiar \textit{n}-grams.

% % We notice that despite high style, hybrid, and topical similarity on \blogsmall{} and \blogbig{} datasets, we achieved significant performance gain. In contrast, \turingbench{} shows high content similarity but the performance improvement is relatively marginal. We hypothesize that our contrastive learning approach is more effective to distinguish similar texts interpreted by style, hybrid, and topical features. However, it might fall short when the content feature is similar. This is because our contrastive objective \eqnref{eqn:cl_term} is applied to the sentence embeddings $\phi(\cdot)$. This does not lead to significant information gain if the sentences are already similar measured by n-gram frequencies.

% % \textbf{Does LDA or NLG work?} Latent Dirichlet Allocation (LDA) is often used to model topic distributions of human writings \citep{topic_or_style}. 

% \textbf{Inadequacy of NLG models?} We also note the high topical dissimilarity of \turingbench{}. This is unexpected, since every NLG model was given the same set of input prompts when the dataset was constructed (\secref{sect:results_nlg_setup}). Following \citet{topic_or_style}, we model topical similarity using Latent Dirichlet Allocation (LDA; \citealp{lda}). LDA represents a text as a distribution over latent topics, where each topic is represented as a distribution over words. This observation suggests that some NLG models may struggle to write on topic.\footnote{See \appendixref{sec:nlg_sample_analysis} for a brief analysis.} Nevertheless, Contra-X still provides an improvement over the baseline, showing its generality across text of varying quality. %although it is also possible that LDA is less suitable for modeling topical differences on neural-generated text.

% % Here is another interesting observation. As described in \secref{sect:results_nlg_setup}, \turingbench{} is constructed by querying the machine authors to write about the same set of titles. This is to reduce the topical difference between authors \citep{turing_benchmark}. However, Latent Dirichlet Allocation (LDA) \citep{lda} reflects high topical dissimilarity on the dataset compared to the others. This either reflects the inadequacy of certain NLG models (\ie{} being unable to write on-topic) or suggests a room for improvement for topical models.

% % a need for a different approach to identifying topics in future work.

% % This suggests that when the authors in a dataset write about highly similar topics, the contrastive learning objective is particularly useful in finding minute difference between authors.

% % In contrast, on the content metric, \turingbench{} shows the greatest similarity. We conjecture that this is correlated to the lack of performance gain from the contrastive models since content similarity measures word n-gram frequencies. Since our contrastive learning objective maximises the difference between learned representations at the word embedding level, a high degree of content similarity may predict the inability of the contrastive model to perform effectively.

% % We note that there are multiple confounders present in this analysis, such as the number of authors in each dataset. Additionally, the feature metrics we use were designed for analysing human-authored text and may not fully capture the nuances of the machine-generated text in \turingbench{}.

% \paragraph{Author-Level Analysis.} Next, we analyze how author characteristics affect model performance on these authors. Specifically, we examine the correlation between the similarity of specific authors and how well the models distinguish between them. We define the distance between two authors to be the mean distance across all representation spaces:

% % Going one step further, we wish to understand how the model performs on distinguishing specific authors in a dataset. Again, we conduct the study in a pairwise manner: we compute the similarity between a pair of authors and correlate it with the predictions that a model make on the authors. We define the distance of two authors as the mean distance across all representation spaces.

% % \begin{equation} \label{pairwise_sim}
% %     d(\mathcal{A}_i, \mathcal{A}_j) = \frac{1}{|F|}\sum_{feat} {\frac{1}{Norm} * Dist(\bar{F}_{feat}^{\mathcal{A}_i}, \\ \bar{F}_{feat}^{\bar{A}_j})}
% % \end{equation} 

% \begin{equation} \label{pairwise_sim}
%     PD(A_i, A_j) = \frac{1}{|\mathcal{F}|} \sum_{f \in \mathcal{F}} \frac{1}{C_f} d(v_{A_i}^f, v_{A_j}^f),
% \end{equation} 

% where $C_f$ is a normalization term, defined as 

% % where $Norm$ is the normalization term

% % \begin{equation} \label{pairwise_sim}
% %     Norm = {\max\limits_{m, n \in D}{(Dist(\bar{F}_{feat}^{\mathcal{A}_m}, \\ \bar{F}_{feat}^{\bar{A}_n}))}}
% % \end{equation} 

% % We conjecture that when two authors are highly similar, contrastive learning models can achieve improved class-level performance on those authors over a baseline model which may struggle to differentiate the two.

% \begin{equation}
%     C_f = \max_{A_i, A_j \in \mathcal{D}} d(v_{A_i}^f, v_{A_j}^f).
% \end{equation}

% \begin{figure}[t!]
%     \small
%     \centering
%     \begin{subfigure}{\columnwidth}
%         \includegraphics[width=\columnwidth]{figs/pair_feat_300dpi_numbered.png}
%         \caption{Feature dissimilarity matrix. Darker is more similar.}\label{fig:feature_matrix}
%     \end{subfigure}
%     \begin{subfigure}{\columnwidth}
%     \includegraphics[width=\columnwidth]{figs/pair_cm_300dpicolor_numbered.png}
%     \caption{Relative confusion matrix. This is obtained by subtracting the confusion matrix of \bertbase{} from that of \bertcl{}.}\label{fig:confusion}
%     \end{subfigure}
%     \caption{Feature similarity matrix and relative confusion matrix between \bertbase{} and \bertcl{} on selected authors. In both figures, $(i, j)$ denotes the cell at the $i$-indexed row and $j$-indexed column. In (\subfig{a}), $(i, j)$ denotes $d(A_i, A_j)$, the feature dissimilarity between the two authors. In (\subfig{b}), a lower value (blue) of $(i, j)$ indicates \bertcl{} confused \Ai{} for \Aj{} less than \bertbase{}.}
%     \label{fig:pair_cm_300}
% \end{figure}

% We plot the similarity matrix for selected \blogbig{} authors in \figref{fig:feature_matrix}. The authors are selected such that they form pairs that are highly indistinguishable by the above metrics, as well as t-SNE clustering and human inspection. The cells numbered 1-4 represent the most similar author pairs (\ie{} darker-coloured cells). Performance-wise, on each of these pairs, \bertcl{} shows significant improvements in overall class-level accuracy over \bertbase{}.\footnote{See \appendixref{sec:bert_similar_appendix} for exact values. This trend also holds for \debertacl{} and \debertabase{}; see \appendixref{sec:deberta_similar_appendix}.} This is consistent with the intuition that contrastive learning is more useful for distinguishing author pairs that are more similar.

% % \figref{fig:pair_cm} shows selected authors from the \blogbig{} dataset. The left matrix shows the mean normalized similarities  across the four features $\bar{F}_{feat}^{\textit{A}}$ between authors (darker squares represent greater similarities). The squares numbered 1-4 represent the most similar author pairs.

% \textbf{Increased bias.} The pairwise improvement mentioned above shows a curious property of being biased towards one of the authors in the pair. To visualize this, we subtract the confusion matrix of \bertbase{} from that of \bertcl{} and name the result the \textit{relative confusion matrix} (\figref{fig:confusion}). Each cell in the matrix indicates the increase in the probability that an author $A_i$ is classified as $A_j$ from \bertbase{} to \bertcl{}. For example, the blue cell at $(12, 43)$ shows that \bertcl{} confused $A_{12}$ as $A_{43}$ less than \bertbase{}, while the orange cell at $(43, 12)$ shows that \bertcl{} confused $A_{43}$ as $A_{12}$ more frequently.

% %  the other. The colour of a given cell $(i, j)$, $i \neq j$, indicates whether \bertcl{} confused \Aj{} for \Ai{} more or less often than \bertbase{}. 

% % which model confused \Aj{} for \Ai{} more often. For instance, the light-coloured $(43, 12)$ shows that \bertbase{} confused $A_{12}$ as $A_{43}$ more than \bertcl{}, while the darker $(12, 43)$ shows that \bertcl{} confused $A_{43}$ as $A_{12}$ more often.

% % For instance, the light-coloured $(12, 43)$ shows that \bertbase{} misclassified 156 more samples of $A_{12}$ as $A_{43}$ than \bertcl{}, while the darker colour of $(43, 12)$ shows that \bertcl{} wrongly classified 131 more samples of $A_{43}$ as $A_{12}$.

% Note first the intuitive link between the similarity and confusion matrices: similar authors are more likely to be confused by one of the models for each other. Observe also that the pairs in the confusion matrix are always present in light-dark pairs. In other words, if \bertbase{} misclassifies more samples from \Ai{} as \Aj{} (\eg{} $A_{12}$ as $A_{43}$), then \bertcl{} mislabels more samples from \Aj{} as \Ai{} (\ie{} $A_{43}$ as $A_{12}$). This suggests that \bertcl{} trades the ability to identify \Aj{} samples for classifying \Ai{} samples better. Note that this observation is unlikely to be due to class imbalance, as \Ai{} and \Aj{} contain similar numbers of samples.\footnote{See \appendixref{sec:bert_similar_appendix} for exact sample counts.}

% % The baseline models \bertbase{} and \debertabase{} systematically misclassify certain authors as other highly similar authors. With the addition of the contrastive learning objective, the models achieve a substantial increase in overall accuracy while systematically misclassifying a different set of authors. 

% Nevertheless, the cumulative accuracy across \Ai{} and \Aj{} is always higher for \bertcl{} compared to the baseline, \eg{} 33.6\% vs 23.1\% for $A_{12}$ and $A_{43}$ combined, leading to an overall performance improvement on the whole dataset. This shows that the model implicitly learns to make trade-offs to optimize the contrastive objective, \ie{} it chooses to learn specialized representations that are particularly biased against some authors but improve the average performance over all authors. This shows that \method{} captures certain features that let the model distinguish a subset of the authors. It remains unclear to us whether it is possible to find a representation that yields improvements on all authors across all datasets \footnote{For a similar question, we refer to the No Free Lunch Theorem \citep{no_free_lunch}.}, and we hope our analysis might be a starting point for future investigation. 

% % However, to obtain consistent improvement, we need a deeper understanding of the difference between easily-confused authors and incorporate that insight into the contrastive learning algorithm \citep{no_free_lunch}. However, this is beyond the scope of our paper and we leave it to future work.

% % This might be achieved by constructing more meaningful negative samples. 

% \section{Conclusion} \label{sec:conclusion}
% Successful authorship attribution necessitates the modeling of author-specific characteristics and idiosyncrasies. In this work, we propose to integrate contrastive learning with supervsed learning to tackle this challenge. We demonstrate empirical improvements in authorship attribution on both human-written and machine-generated texts and we also show the generality of the method across different writers, dataset qualities, and dataset sizes. Critically, we contributed analyses of how and when Contra-X works. At the dataset level, we qualitatively showed that \method{} creates a tighter representation spread of each author and increased separation between authors. Within each dataset, at the author level, we found that Contra-X is able to distinguish between highly similar author pairs, trading predictive accuracy on some authors for the overall performance. These analyses help us understand our approach and identify important questions for future work. 

% % The understanding might shed light  Resolving these issues is a direction for further work as this would lead to better overall improvement and increased fairness of the final representation. 


% \clearpage

% \section*{Ethical Considerations}\label{sec:ethical}

% In this subsection, we discuss potential ethical concerns related to the previous discussion on the increased bias in author-level performance.

% \paragraph{Decreased Fairness?} With classification models, fairness in predictions across classes is an important consideration. We want to, for instance, avoid demographic bias \citep{demographic_fairness}, which may manifest as systematic misclassifications of authors with specific sociolinguistic backgrounds.

% % For instance, a model that predicts recidivism rates should not mispredict the outcome for some racial groups more than others \citep{recidivism}. In other words, it is undesirable for a model to show uneven performance across different classes.

% Having observed increased bias against certain authors, we seek to find out if this trend holds across the entire dataset. We quantitatively evaluate this by computing the variance in class-level accuracy across all authors. The results show that the improvements from our contrastive learning objective appear to incur a penalty in between-author fairness. \bertcl{} on \blogsmall{} and \blogbig{}, and \debertacl{} on \blogbig{} achieve substantial gains in accuracy, and also produce notably higher variance than their baseline counterparts.\footnote{See \appendixref{sec:full_class_variance} for exact values.} In contrast, for models where the improvements are marginal, the differences in variance are insignificant. A potential direction for future work is investigating whether the use of contrastive learning consistently exacerbates variances in class-level accuracy. Studying the characteristics of the classes that the model is biased against may boost not just overall performance, but also predictive fairness.

% % we notice that across all datasets, \bertcl{} and \debertacl{} systematically exhibit a higher variance in class-level accuracy than \bertbase{} and \debertabase{} respectively (\tabref{table:class_variance}). This disparity is positively correlated to the overall accuracy improvement from the contrastive model. In classification models, class-level accuracy imbalance is potentially an undesirable trait in real-world applications for reasons of fairness. (For example, a model that predicts recidivism rates should not mispredict the outcome for some racial groups more than others.) Due care should therefore be exercised in this matter.

% % We note a curious property exhibited by the contrastive learning models. When a baseline model consistently misclassifies samples from an author \textit{$A_i$} as being from a highly similar author \textit{$A_j$}, the corresponding contrastive model often shows the opposite behaviour of correctly classifying \textit{$A_i$} samples, while mislabelling \textit{$A_j$} samples as being from \textit{$A_i$}. 

% % \figref{fig:pair_cm} shows selected author pairs on the \blogbig{} dataset. The left matrix shows the relative performance of \bertbase{} and \bertcl{}. The light-dark pairs about the main diagonal indicate that where \bertbase{} confused \textit{$A_i$} for \textit{$A_j$}, \bertcl{} confused \textit{$A_j$} for \textit{$A_i$}. The right matrix shows the mean normalized similarity between author pairs across the four feature metrics. Note how the darker squares (indicating similar authors) correspond to the light-dark pairs in the left matrix.

% % This trend of "sacrificing" accuracy for one author \textit{$A_j$} in favour of another \textit{$A_i$} is also present in \debertacl{} on \blogbig{} and \bertcl{} on \blogsmall{}. We note that in doing so, the cumulative accuracy across both authors in the pair is always higher for the contrastive learning model than its baseline counterpart, which contributes to the better overall performance of the contrastive model. Nevertheless, this motivates future work to find a better algorithm that improves performance on \textit{$A_j$} without doing significantly worse on \textit{$A_i$}.

% % The contrastive learning objective works well to differentiate authors with similar representations. Authors 46 and 48 both see improvements

% % $0.0177$, $0.00046$ $2.2%$ $84.7\%$

% % Empirically, the separation effect leads to performance improvement of \bertcl{}. For the \bertbase{} approach,  vectors are mixed up (i.e. class 5, 6, and 9). The clustering directly reflects the accuracy as it corresponds well with the confusion matrix in Figure XXX, where it can be observed that some classes (i.e. class 5) are more accurately predicted with the proposed method.

% % present the visualization of representative features learned by the proposed model and the baseline model, to illustrate the effectiveness of contrastive learning. To visualize the representations, we apply t-SNE and PCA on embeddings of samples from the test set, by reducing the high-dimensional vectors and projecting them onto a 2-dimensional space. We take the dataset Blog (with 10 authors) for example, apply both out proposed model (with L2) and the baseline model, and plot the clusterings in Figure XXX (TODO: use a/b s62B). The learned representative features of different authors are generally clearly separated, due to L2's power to drag samples from different classes away from each other. In contrast, vectors are mixed up with the baseline approach (i.e. class 5, 6, and 9). The clustering directly reflects the accuracy as it corresponds well with the confusion matrix in Figure XXX, where it can be observed that some classes (i.e. class 5) are more accurately predicted with the proposed method.

% \clearpage


% % Entries for the entire Anthology, followed by custom entries
% \bibliography{references}
% \bibliographystyle{acl_natbib}

% \clearpage

% \appendix
% \label{sec:appendix}

% \section{Dataset Statistics} \label{sect:statistics}
% \tabref{table:statistics} presents statistics of the \blogsmall{}, \blogbig{}, \imdb{}, and \turingbench{} datasets.

% \section{Effect of Collection Imbalance}
% \label{sec:imbalance}

% For each class $C$, we calculate the \textit{\method{} delta},

% \begin{equation} \label{contrax_difference}
%     \frac{\Delta{}correct}{|C|}
% \end{equation} 

% where $\Delta{}correct$ is the number of samples in $C$ correctly classified by only the contrastive model minus the number of samples correctly classified by only the baseline model. This gives an indication of whether the contrastive model performed better or worse than the baseline on $C$.

% \tabref{table:contradiff_correl} shows the correlation between the \method{} delta and class size. The correlation is near zero in all instances, showing that \method{} does not perform differently on larger or smaller classes compared to the baseline.

% \begin{table}[h]
% %\vspace{-0.25in}
% \centering
% \begin{tabular}{c c c}
%   \toprule
%   \textbf{Model} & \textbf{Dataset} & \textbf{Correlation} \\
%   \midrule
%   \multirow{2}{*}{BERT} & \blogsmall{} & -0.01696 \\
%   & \blogbig{} & 0.02905 \\
%   \multirow{2}{*}{DeBERTa} & \blogsmall{} & -0.01601 \\
%   & \blogbig{} & 0.00707 \\
%   \bottomrule
% \end{tabular}
% \caption{Correlation between \method{} delta and class size. We exclude \turingbench{} from this analysis as the imbalance ratio is small (1:1.12) which makes the correlation unrepresentative.}
% \label{table:contradiff_correl}
% \end{table}

% \section{Similarity Metrics}
% \label{sec:similarity_metrics}

% Following \citet{topic_or_style}, we use four key metrics to analyze the characteristics of individual datasets (\ie{} samples written by a particular author, or all samples in a corpus). We describe these metrics in detail below:

% \textbf{Content.} We measure the frequencies of the most common word unigrams, bigrams, and trigrams to produce a feature vector that represents an author's content preferences over each document.

% \textbf{Style.} We combine multiple stylometric features, \ie{} average word length, number of short words, percentage of digits, percentage of upper-case letters, letter frequency, digit frequency, vocabulary richness, and frequencies of function words and punctuation, into a feature vector representing an author's writing style in a given document.

% \textbf{Hybrid.} We measure the frequencies of the most common character bigrams and trigrams, to capture both content and style preferences of the author \citep{char_ngram} in a given document.

% \textbf{Topic.} We use Latent Dirichlet Allocation (LDA) to generate a probability distribution over an author's possible topics. We run LDA with 20 topics, as in \citet{topic_or_style}, and fit the data over 500 iterations.

% \section{\turingbench{} Dataset Analysis}
% \label{sec:nlg_sample_analysis}

% Closer examination of the \turingbench{} dataset reveals that some models appear to produce fairly incoherent text. \tabref{table:nlg_samples} contains snippets from various models. Qualitatively, it is difficult to identify what the topic of each text is supposed to be; there appear to be multiple topics referenced in each text. This suggests that some of these models do not write on-topic, and so may explain why LDA reflects high topical dissimilarity between models.

% On the other hand, at the phrase level, these models largely put out sensible phrases, \eg{} ``strong economic growth'', ``stunning game'', ``suspicious clicks''. We hypothesize that this explains the comparatively higher content similarity on \turingbench{}, since the content metric measures word \textit{n}-gram frequencies.

% \section{Class-Level Accuracy Variance}
% \label{sec:full_class_variance}
% \tabref{table:class_variance} shows the exact class-level accuracy variances for our four models on \blogsmall{}, \blogbig{}, and \turingbench{}.


% \clearpage

% %\vspace{-0.2in}
% \begin{table*}[t!]
% %\vspace{-0.25in}
% \centering
% \begin{tabular}{c c c c c c}
%   \toprule
%     & \blogsmall{} & \blogbig{} & \imdb{} & \turingbench\\
%   \midrule
%   \# authors & 10 & 50 & 62 & 20\\
%   \# total documents & 23498 & 73275 & 61973 & 149561\\
%   avg char / doc (no whitespace) & 407 & 439 & 1401 & 1063\\
%   avg words / doc & 118 & 124 & 341 & 188\\
%   \bottomrule
% \end{tabular}
% \caption{Statistics of the four datasets used in our experiments.}
% \label{table:statistics}
% \end{table*}

% \begin{table*}

% \centering
% \begin{tabular}{p{0.25\linewidth} | p{0.7\linewidth}}
%   \toprule
%   \textbf{Model} & \textbf{Text} \\
%   \midrule
%   CTRL & ``apple gives tim cook \$384 million stock grant... steve jobs is set to receive an additional \$1.4 billion in cash... recovery needs but it also requires p le with skills not just on paper or through education training but, crucially, real work experience. those are two things which can only come if we have strong economic growth...''\\
%   FAIR\_WMT19 & ``antoine helps real sociedad draw with valladolid... sociedad's goal in a 1-1 was highlight of stunning game played on night terrorist bombing attack manchester. tuesday, two bombs exploded central manchester arena during popular outdoor concert, killing 22 p le and injuring hundreds more..."\\
%   GROVER\_MEGA & ``...the messages, which along message some will choose avoid draft, ready for qualification training are fake, according public affairs. do not respond spoof, requires suspicious clicks, pictures, or notes function, an official memo from issued thursday reads...''\\
%   TRANSFORMER\_XL & ``carlos ghosn, mum on tokyo escape, unleashes a rambling defense of the state student-teacher training program in japan... as 2015, three universities (hiroshima, izumo, kawachi) accept all two degrees; they have also accepted each other. nevertheless, buddhist monks maintain that their colleges provide admission hindu traditions rather than admitting any religious instruction.''\\
%   \midrule
% \end{tabular}
% \caption{Sample text snippets from various NLG models in the \turingbench{} dataset. }
% \label{table:nlg_samples}
% % \vspace{3in}
% \end{table*}

% \begin{table*}
%     \centering
%     %\vspace*{-1.1in}
%     \begin{tabular}{c c c c}
%     \toprule
%      & \textbf{\blogsmall{}} & \textbf{\blogbig{}} & \textbf{\turingbench{}} \\
%     \midrule
%     \bertbase{} & 0.15494 & 0.10430 & 0.06747 \\
%     \bertcl{} & \textbf{0.17698} (Acc. +5.9) & \textbf{0.12087} (Acc. +6.8) & \textbf{0.06772} (Acc. +1.43) \\
%     % Acc. {$\uparrow$} & 5.9 & 6.8 & 1.13 \\
%     \midrule
%     \debertabase{} & 0.19735 & 0.13267 & \textbf{0.05191} \\
%     \debertacl{} & \textbf{0.20029} (Acc. +1.7) & \textbf{0.14343} (Acc. +3.7) & 0.05126 (Acc. +0.73) \\
%     % Acc. {$\uparrow$} & 0.6 & 3.7 & 0.53 \\
%     \bottomrule
%     \end{tabular}
%     \caption{Variance in class-level accuracy (accuracy increase by each contrastive model is listed for reference). The higher the variance, the more the model performance varies between different classes. For each dataset, higher variance for each baseline/contrastive pair is \textbf{bolded}.}
%     \vspace*{0.75in}
%     \label{table:class_variance}
% \end{table*}

% \clearpage

% % %\vspace{-2in}
% % \begin{table*}[t]
% % \centering
% % \begin{tabular}{c c c c c}
% %   \toprule
% %   Model & \blogsmall{} & \blogbig{} & \imdb{} \\
% %   \midrule
% %   Token SVM \citep{imdb62} & - & - & 92.5 \\
% %   Char-CNN \citep{char_cnn} & 61.2 & 49.4 & 91.7 \\
% %   Continuous N-gram \citep{conti_ngram} & 61.3 & 52.8 & 95.1 \\
% %   N-gram CNN \citep{ngrams_cnn} & 63.7 & 53.1 & 95.2 \\
% %   Syntax CNN \citep{syntax_cnn} & 64.1 & 56.7 & \textbf{96.2} \\
% %   BertAA \citep{bertaa} & \textbf{65.4} & \textbf{59.7} & 93.0 & \\ 
% %   \midrule
% %   \bertbase{} & 60.3 & 55.6 & 97.2\\
% %   \bertcl{} & 66.0 (5.7\textcolor{black}{$\uparrow$}) & 62.2(6.6\textcolor{black}{$\uparrow$}) & 97.7(0.5\textcolor{black}{$\uparrow$})\\
% %   \debertabase{} & 68.0 & 65.0 & 98.1\\
% %   \textbf{\debertacl{}} & \textbf{69.9(1.9\textcolor{black}{$\uparrow$})} & \textbf{69.7(4.7\textcolor{black}{$\uparrow$})} & \textbf{98.2(0.1\textcolor{black}{$\uparrow$})}\\
% %   \bottomrule
% % \end{tabular}
% % \caption{Results of human authorship attribution - 8:2 train/test split}
% % \label{table:result_82}
% % \end{table*}


% % \section{Human Authorship Attribution Results with 8:2 Split} \label{sect:result82}
% % Following \citet{bertaa}, we divide the datasets into train-test splits at an 8:2 ratio for \blogsmall{}, \blogbig{}, and \imdb{} and follow the default split for \turingbench. We show the results on the test set in \tabref{table:result_82}. 

% \section{Analysis of Similar Author Pairs}
% \label{sec:similar_authors}

% \subsection{\bertbase{} and \bertcl{}}
% \label{sec:bert_similar_appendix}

% \figref{fig:pair_feat_cm_individual} shows the individual similarity matrices for the four feature types. The general pattern of the highlighted pairs being darker (\ie{} more similar) than their surrounding cells can be seen across all the matrices. \tabref{table:bert_blog50_pairs} shows the exact prediction accuracies for the four highlighted pairs. As noted previously, \bertcl{} always achieves a higher total accuracy (defined as total correct predictions over total samples) over both authors in a pair compared to \bertbase{}. 

% \subsection{\debertabase{} and \debertacl{}}
% \label{sec:deberta_similar_appendix}

% \figref{fig:pair_2_cm} shows the feature similarity matrices and the relative confusion matrix for selected authors for \debertabase{} and \debertacl{}. Note that some of the author pairs are the same as those shown for \bertbase{} (\ie{} 6 \& 44, 38 \& 39) while other pairs are different. Similar to \figref{fig:pair_cm_300}(\subfig{b}), the colour of a given cell $(i, j)$, $i \neq j$, indicates whether \debertacl{} confused \Ai{} for \Aj{} more or less often than \debertabase{}. For instance, the blue-coloured $(1, 15)$ shows that \debertacl{} confused $A_{1}$ as $A_{15}$ less than \debertabase{}, while the orange $(15, 1)$ shows that \debertacl{} confused $A_{15}$ as $A_{1}$ more times.

% \tabref{table:deberta_blog50_pairs} shows the exact prediction accuracies for the highlighted pairs. As with \bertcl{}, \debertacl{} achieves a higher total accuracy on each pair than \debertabase{}.

% % \figref{fig:pair_2_feat_cm_individual} shows the individual similarity matrices for the four feature types.

% % \section{Full \turingbench{} results}
% % \label{sec:full_turing_results}
% % \tabref{table:sota_nlg_full} shows the precision, recall, F1, and accuracy scores on \turingbench{}.

% \clearpage

% \begin{figure*}[h!]
%     \centering
%     \includegraphics[width=0.9\columnwidth]{figs/pair_content_300dpi_numbered.png}
%     \includegraphics[width=0.9\columnwidth]{figs/pair_topic_300dpi_numbered.png}
%     \includegraphics[width=0.9\columnwidth]{figs/pair_hybrid_300dpi_numbered.png}
%     \includegraphics[width=0.9\columnwidth]{figs/pair_style_300dpi_numbered.png}
%     \caption{(Clockwise from top left) Similarity metrics between authors \Ai{} ($i$-indexed row) and \Aj{} ($j$-indexed column) for content, topic, hybrid, and style features respectively for selected authors on \blogbig{}.}
%     \label{fig:pair_feat_cm_individual}
% \end{figure*}

% \begin{table*}
%     \centering
%     %\vspace*{-1.35in}
%     \begin{tabular}{c | c c c | c c c | c }
%       \hline
%       & \multicolumn{3}{c|}{\textbf{Author 1}} & \multicolumn{3}{c|}{\textbf{Author 2}} & Total \\
%       Model & \# & Samples & Correct & \# & Samples & Correct & Accuracy (\%) \\
%       \hline \bertbase{} & \multirow{2}{*}{12} & \multirow{2}{*}{229} & 2 & \multirow{2}{*}{43} & \multirow{2}{*}{225} & 47 & 10.8 \\
%       \bertcl{} & & & 209 & & & 0 & \textbf{46.0} \\
%       \hline \bertbase{} & \multirow{2}{*}{30} & \multirow{2}{*}{153} & 8 & \multirow{2}{*}{26} & \multirow{2}{*}{154} & 92 & 32.6 \\
%       \bertcl{} & & & 135 & & & 0 & \textbf{44.0} \\
%       \hline \bertbase{} & \multirow{2}{*}{6} & \multirow{2}{*}{116} & 35 & \multirow{2}{*}{44} & \multirow{2}{*}{113} & 18 & 23.1 \\
%       \bertcl{} & & & 73 & & & 4 & \textbf{33.6} \\
%       \hline \bertbase{} & \multirow{2}{*}{38} & \multirow{2}{*}{112} & 48 & \multirow{2}{*}{39} & \multirow{2}{*}{112} & 8 & 25.0 \\
%       \bertcl{} & & & 96 & & & 0 & \textbf{42.9} \\
%       %\bertcl{} & 12 & 229 & 209 & 43 & 225 & 0 & \textbf{46.0} \\
%     %   \hline \bertbase{} & 30 & 153 & 8 & 26 & 154 & 92 & 32.6 \\
%     %   \bertcl{} & 30 & 153 & 135 & 26 & 154 & 0 & \textbf{44.0} \\
%     %   \hline \bertbase{} & 6 & 116 & 35 & 44 & 113 & 18 & 23.1 \\
%     %   \bertcl{} & 6 & 116 & 73 & 44 & 113 & 4 & \textbf{33.6} \\
%     %   \hline \bertbase{} & 38 & 112 & 48 & 39 & 112 & 8 & 25.0 \\
%     %   \bertcl{} & 38 & 112 & 96 & 39 & 112 & 0 & \textbf{42.9} \\
%       \hline
%     \end{tabular}
%     \caption{Performance of \bertbase{} and \bertcl{} on selected author pairs of \blogbig{}. Higher accuracy for each pair is \textbf{bolded}.}
%     %\vspace*{1in}
%     \label{table:bert_blog50_pairs}
%     \vspace*{1.6in}
% \end{table*}

% \clearpage

% % \begin{table*}[t]
% % \centering
% % \begin{tabular}{c c c c c}
% %   \toprule
% %   \textbf{Model} & \textbf{Precision} & \textbf{Recall} & \textbf{F1} & \textbf{Accuracy} \\
% %   \midrule
% %   Random Forest & 58.93 & 60.53 & 58.47 & 61.47 \\
% %   SVM (3-grams) & 71.24 & 72.23 & 71.49 & 72.99 \\
% %   WriteprintsRFC & 45.78 & 48.51 & 46.51 & 49.43 \\
% %   OpenAI detector\footnote{\url{https://huggingface.co/roberta-base-openai-detector}} & 78.10 & 78.12 & 77.14 & 78.73 \\
% %   Syntax CNN & 65.20 & 65.44 & 64.80 & 66.13 \\
% %   N-gram CNN & 69.09 & 68.32 & 66.65 & 69.14 \\
% %   N-gram LSTM-LSTM & 6.694 & 68.24 & 66.46 & 68.98 \\
% %   BertAA & 77.96 & 77.50 & 77.58 & 78.12 \\ 
% %   BERT & 80.31 & 80.21 & 79.96 & 80.78 \\
% %   RoBERTa & 82.14 & 81.26 & 81.07 & 81.73 \\
% %   \midrule
% %   \bertbase{} \textit{(our baseline)} & 78.56 & 78.81 & 78.53 & 79.46 \\
% %   \bertcl{} & 80.10 (1.66\textcolor{black}{$\uparrow$}) & 79.99 (1.88\textcolor{black}{$\uparrow$}) & 79.84 (1.31\textcolor{black}{$\uparrow$}) & 80.59 (1.13\textcolor{black}{$\uparrow$})\\
% %   \debertabase{} \textit{(our baseline)} & 82.16 & 81.84 & 81.82 & 82.00 \\
% %   \textbf{\debertacl{}} & \textbf{82.84 (0.68\textcolor{black}{$\uparrow$})} & \textbf{82.04 (0.20\textcolor{black}{$\uparrow$})} & \textbf{81.98 (0.17\textcolor{black}{$\uparrow$})} & \textbf{82.53 (0.53\textcolor{black}{$\uparrow$})}\\
% %   \bottomrule
% % \end{tabular}
% % \caption{Full results across four metrics on human and machine authorship attribution. Results in top section are from the \turingbench\ paper. Improvements over the baselines are indicated in parentheses. Best model is \textbf{bolded}. }
% % \label{table:sota_nlg_full}
% % \end{table*}

% %\newpage
% \begin{figure*}[t]
%     \centering\
%     % \hspace*{-0.1in}
%     \includegraphics[width=\columnwidth]{figs/pair2_feat_300dpi_numbered.png}
%     \includegraphics[width=\columnwidth]{figs/pair2_cm_300dpicolor_numbered.png}\\
%     \small(\subfig{a}) Feature similarity matrix (left) and relative confusion matrix (right) between \debertabase{} and \debertacl{} on selected authors. For both figures, $(i, j)$ denotes the cell at the $i$-indexed row and $j$-indexed column. In the similarity matrix, $(i, j)$ denotes $d(A_i, A_j)$, the dissimilarity between the two authors (darker = more similar). In the confusion matrix, a lower value of $(i, j)$ indicates \debertacl{} confused \Ai{} for \Aj{} less than \debertabase{}.\\
%     % $(i, j)$ denotes whether \debertacl{} confused \Ai{} for \Aj{} more (lighter) or less (darker) than \debertabase{}
%     \vspace{0.5in}
%     \includegraphics[width=\columnwidth]{figs/pair2_content_300dpi_numbered.png}
%     \includegraphics[width=\columnwidth]{figs/pair2_topic_300dpi_numbered.png}
%     \includegraphics[width=\columnwidth]{figs/pair2_hybrid_300dpi_numbered.png}
%     \includegraphics[width=\columnwidth]{figs/pair2_style_300dpi_numbered.png}\\
%     \small(\subfig{b}) (Clockwise from top left) Similarity metrics between authors \Ai{} ($i$-indexed row) and \Aj{} ($j$-indexed column) for content, topic, hybrid, and style features respectively for selected authors on \blogbig{}.\\
%     \caption{Visualizations for selected author pairs for \debertabase{} and \debertacl{} on \blogbig{}.}
%     \vspace*{0.5in}
%     \label{fig:pair_2_cm}
% \end{figure*}

% \clearpage

% \begin{table*}[t]
% \centering
% %\vspace*{-2.5in}
% \begin{tabular}{c | c c c | c c c | c }
%   \hline
%   & \multicolumn{3}{c|}{\textbf{Author 1}} & \multicolumn{3}{c|}{\textbf{Author 2}} & Total \\
%   Model & \# & Samples & Correct & \# & Samples & Correct & Accuracy (\%) \\
%   \hline \debertabase{} & \multirow{2}{*}{1} & \multirow{2}{*}{109} & 0 & \multirow{2}{*}{15} & \multirow{2}{*}{103} & 94 & 44.3 \\
%   \debertacl{} & & & 107 & & & 0 & \textbf{50.5} \\
%   \hline \debertabase{} & \multirow{2}{*}{47} & \multirow{2}{*}{105} & 0 & \multirow{2}{*}{48} & \multirow{2}{*}{104} & 61 & 29.2 \\
%   \debertacl{} & & & 102 & & & 4 & \textbf{50.7} \\
%   \hline \debertabase{} & \multirow{2}{*}{44} & \multirow{2}{*}{113} & 24 & \multirow{2}{*}{6} & \multirow{2}{*}{116} & 28 & 22.7 \\
%   \debertacl{} & & & 108 & & & 3 & \textbf{48.5} \\
%   \hline \debertabase{} & \multirow{2}{*}{38} & \multirow{2}{*}{112} & 0 & \multirow{2}{*}{39} & \multirow{2}{*}{112} & 90 & 40.2 \\
%   \debertacl{} & & & 81 & & & 12 & \textbf{41.5} \\
%   %\bertcl{} & 12 & 229 & 209 & 43 & 225 & 0 & \textbf{46.0} \\
% %   \hline \bertbase{} & 30 & 153 & 8 & 26 & 154 & 92 & 32.6 \\
% %   \bertcl{} & 30 & 153 & 135 & 26 & 154 & 0 & \textbf{44.0} \\
% %   \hline \bertbase{} & 6 & 116 & 35 & 44 & 113 & 18 & 23.1 \\
% %   \bertcl{} & 6 & 116 & 73 & 44 & 113 & 4 & \textbf{33.6} \\
% %   \hline \bertbase{} & 38 & 112 & 48 & 39 & 112 & 8 & 25.0 \\
% %   \bertcl{} & 38 & 112 & 96 & 39 & 112 & 0 & \textbf{42.9} \\
%   \hline
% \end{tabular}
% \caption{Performance of \debertabase{} and \debertacl{} on selected author pairs of \blogbig{}. Higher accuracy for each pair is \textbf{bolded}.} 
% \vspace*{7in}
% %\vspace*{0.15in}
% \label{table:deberta_blog50_pairs}
% \end{table*}

% % \begin{figure*}[ht!]
% %     \centering
% %     \includegraphics[width=0.9\columnwidth]{figs/pair_2_content_cm_numbered.png}
% %     \includegraphics[width=0.9\columnwidth]{figs/pair_2_topic_cm_numbered.png}
% %     \includegraphics[width=0.9\columnwidth]{figs/pair_2_hybrid_cm_numbered.png}
% %     \includegraphics[width=0.9\columnwidth]{figs/pair_2_style_cm_numbered.png}
% %     \caption{(Clockwise from top left) Similarity metrics for content, topic, hybrid, and style respectively for selected authors for \debertabase{} and \debertacl{} on \blogbig{}. }
% %     \label{fig:pair_2_feat_cm_individual}
% % \end{figure*}

% % \newpage
% % \begin{table*}
% % \centering
% % \begin{tabular}{c | c c c | c c c | c }
% %   \hline
% %   & \multicolumn{3}{c|}{Author 1} & \multicolumn{3}{c|}{Author 2} & Total \\
% %   Model & \# & Samples & Correct & \# & Samples & Correct & Accuracy (\%) \\
% %   \hline \debertabase{} & \multirow{2}{*}{1} & \multirow{2}{*}{109} & 0 & \multirow{2}{*}{15} & \multirow{2}{*}{103} & 94 & 44.3 \\
% %   \debertacl{} & & & 107 & & & 0 & \textbf{50.5} \\
% %   \hline \debertabase{} & \multirow{2}{*}{47} & \multirow{2}{*}{105} & 0 & \multirow{2}{*}{48} & \multirow{2}{*}{104} & 61 & 29.2 \\
% %   \debertacl{} & & & 102 & & & 4 & \textbf{50.7} \\
% %   \hline \debertabase{} & \multirow{2}{*}{44} & \multirow{2}{*}{113} & 24 & \multirow{2}{*}{6} & \multirow{2}{*}{116} & 28 & 22.7 \\
% %   \debertacl{} & & & 108 & & & 3 & \textbf{48.5} \\
% %   \hline \debertabase{} & \multirow{2}{*}{38} & \multirow{2}{*}{112} & 0 & \multirow{2}{*}{39} & \multirow{2}{*}{112} & 90 & 40.2 \\
% %   \debertacl{} & & & 81 & & & 12 & \textbf{41.5} \\
% %   %\bertcl{} & 12 & 229 & 209 & 43 & 225 & 0 & \textbf{46.0} \\
% % %   \hline \bertbase{} & 30 & 153 & 8 & 26 & 154 & 92 & 32.6 \\
% % %   \bertcl{} & 30 & 153 & 135 & 26 & 154 & 0 & \textbf{44.0} \\
% % %   \hline \bertbase{} & 6 & 116 & 35 & 44 & 113 & 18 & 23.1 \\
% % %   \bertcl{} & 6 & 116 & 73 & 44 & 113 & 4 & \textbf{33.6} \\
% % %   \hline \bertbase{} & 38 & 112 & 48 & 39 & 112 & 8 & 25.0 \\
% % %   \bertcl{} & 38 & 112 & 96 & 39 & 112 & 0 & \textbf{42.9} \\
% %   \hline
% % \end{tabular}
% % \caption{Performance of \debertabase{} and \debertacl{} on selected author pairs of \blogbig{}. Higher accuracy for each pair is \textbf{bolded}.} 
% % \vspace*{7in}
% % \label{table:deberta_blog50_pairs}
% % \end{table*}

% \newpage


% \end{document}

